Recommendation Unlearning

Recommender systems provide essential web services by learning users' personal preferences from collected data. However, in many cases, systems also need to forget some training data. From the perspective of privacy, several privacy regulations have recently been proposed, requiring systems to eliminate any impact of the data whose owner requests to forget. From the perspective of utility, if a system's utility is damaged by some bad data, the system needs to forget these data to regain utility. From the perspective of usability, users can delete noise and incorrect entries so that a system can provide more useful recommendations. While unlearning is very important, it has not been well-considered in existing recommender systems. Although there are some researches have studied the problem of machine unlearning in the domains of image and text data, existing methods can not been directly applied to recommendation as they are unable to consider the collaborative information. In this paper, we propose RecEraser, a general and efficient machine unlearning framework tailored to recommendation task. The main idea of RecEraser is to partition the training set into multiple shards and train a constituent model for each shard. Specifically, to keep the collaborative information of the data, we first design three novel data partition algorithms to divide training data into balanced groups based on their similarity. Then, considering that different shard models do not uniformly contribute to the final prediction, we further propose an adaptive aggregation method to improve the global model utility. Experimental results on three public benchmarks show that RecEraser can not only achieve efficient unlearning, but also outperform the state-of-the-art unlearning methods in terms of model utility. The source code can be found at https://github.com/chenchongthu/Recommendation-Unlearning

==> figs/framework.tex <==

\tikzset{
  FARROW/.style={arrows={-{Latex[length=1.25mm, width=1.mm]}}, thick},
  user/.style = {circle, fill=salmon!72, draw=salmon!400, minimum width=0.8em, align=center, inner sep=0, outer sep=0},
  item/.style = {circle, fill=monte_carlo!72, draw=monte_carlo!400, minimum width=0.8em, align=center, inner sep=0, outer sep=0},
  model/.style = {rectangle, minimum width=2.5em, minimum height=1.8em, align=center, inner sep=2, outer sep=0, font=\normalsize, rounded corners=1},
  data/.style = {rectangle, fill=egg_shell, draw=egg_shell!400, minimum width=1.6cm, minimum height=2.4cm, inner sep=0.3em, rounded corners=4},
}

\begin{figure}
\centering
\resizebox{0.99\linewidth}{!}{
    \begin{tikzpicture}
        
    \node[rectangle, fill=athens_gray, draw, minimum width=12em, minimum height=2em,align=center, inner sep=1.2mm, outer sep=1, rounded corners=2] (o) at (0, 0) {Original training data};
    
    \node[above of=o, node distance=2.5cm, align=center] (p) {\Large $\cdots$};
    \node[item, left of=p, node distance=0.8cm, yshift=0.25cm] (m2i2) {};
    \node[item, left of=p, node distance=0.8cm, yshift=-0.25cm] (m2i3) {};
    \node[item, above of=m2i2, node distance=0.5cm] (m2i1) {};
    \node[item, below of=m2i3, node distance=0.5cm] (m2i4) {};
    \node[user, left of=m2i2, node distance=1cm, yshift=0.2cm] (m2u1) {};
    \node[user, below of=m2u1, node distance=0.5cm] (m2u2) {};
    \node[user, below of=m2u2, node distance=0.5cm] (m2u3) {};
    
    \draw[] (m2u1) -- (m2i2) --(m2u3) -- (m2i1);
    \draw[] (m2u1) -- (m2i3) -- (m2u2) -- (m2i4);
    
    \begin{scope}[on background layer]
     \node [data, fill=chardonnay!42, draw=chardonnay!200, fill opacity=1, fit={(m2u3) (m2i1) (m2i4)}] (s2) {};
     \end{scope}
     
     \foreach \x in {1,2,3,4}
     {
        \node[item, left of=m2i\x, node distance=2.2cm] (m1i\x) {};
     } 
     \node[user, left of=m1i1, node distance=1cm, yshift=-0.25cm] (m1u1) {};
     \node[user, left of=m1i3, node distance=1cm, yshift=-0.25cm] (m1u2) {};
     \draw[] (m1u1) -- (m1i1);
     \draw[] (m1u1) -- (m1i2) -- (m1u2);
     \draw[] (m1u1) -- (m1i3) --(m1u2);
     \draw[] (m1u2) -- node[] (un_edge) {} (m1i4) ;
     
     \begin{scope}[on background layer]
        \node [data, fill=Madang!42, draw=Madang!400, fit={(m1u1) (m1i1) (m1i4)}] (s1) {};
     \end{scope}
     
     
     \node[user, right of=p, node distance=0.8cm] (m3u2) {};
     \node[user, above of=m3u2, node distance=0.6cm] (m3u1) {};
     \node[user, below of=m3u2, node distance=0.6cm] (m3u3) {};
     \foreach \x in {1,2,3}
     {
        \node [item, right of=m3u\x, node distance=1cm] (m3i\x) {};
     } 
     \begin{scope}[on background layer]
        \node [data, fill=fog!42, draw=fog!400, fill opacity=1, fit={(m3u3) (m3i1)}] (s3) {};
     \end{scope}
     
     
     \draw[] (m3u1) -- (m3i1) -- (m3u3) -- (m3i3) -- (m3u2) -- (m3i2) -- (m3u3);
     
     \foreach \x in {1,2,3}
     {
        \node [item, right of=m3i\x, node distance=2.2cm] (m4i\x) {};
     } 
     \foreach \x in {1,2,3,4}
     {
        \node [user, right of=m2i\x, node distance=3.8cm] (m4u\x) {};
     } 
     \draw[] (m4u1) -- (m4i2) -- (m4u3) -- (m4i3) -- (m4u1);
     \draw[] (m4u2) -- (m4i1) -- (m4u4) -- (m4i2);
     \begin{scope}[on background layer]
        \node [data, fill=maya_blue!28, draw=maya_blue!400, fill opacity=1, fit={(m4u1) (m4u4) (m4i1)}] (sK) {};
     \end{scope}
     
     \foreach \x in {1,2,K}
     {
        \node[above of=s\x, node distance=1.4cm, xshift=0.3cm] (sa\x) {\small $S_{\x}$};
     }
     \node[above of=s3, node distance=1.4cm, xshift=0.4cm] (sa3) {\small $S_{K-1}$};
     
     \node [model, fill=Madang!42, draw=Madang!400, above of=s1, node distance=2.4cm] (m1) {$M_{1}$};
     \node [model, fill=chardonnay!42, draw=chardonnay!300, above of=s2, node distance=2.4cm] (m2) {$M_{2}$};
     \node [model, fill=fog!42, draw=fog!400, draw, above of=s3, node distance=2.4cm] (m3) {$M_{K-1}$};
     \node [model, fill=maya_blue!28, draw=maya_blue!400, above of=sK, node distance=2.4cm] (mK) {$M_{K}$};
     \node[above of=p, node distance=2.35cm, align=center] (mdot) {\Large $\cdots$};
     
     \node[rectangle, above of=o, node distance=6.5cm, fill=platinum!80!aluminum, draw, minimum width=12em, minimum height=2em,align=center, inner sep=1.2mm, outer sep=1, rounded corners=2] (agg)  {Attention-based adaptive Aggregation};
      \foreach \x in {1,2,3,K}
     {
        \draw[FARROW] (o.north) -> (s\x.south);
        \draw[FARROW] (s\x.north) -> (m\x.south);
        \draw[FARROW] (m\x.north) -> (agg.south);
     }
     \node[circle, draw, above of=agg, node distance=1.2cm] (output)  {$\times$};
     \draw[FARROW] (agg.north) -> (output.south);
     
     
    \node[left of=output, node distance=3.5cm, align=left] (ma)  {\small$\begin{aligned}
         S_i\!:& ~i\text{-th data shard}\\
         M_i\!:& ~i\text{-th shard model} \\ 
         :& ~\text{data to unlearn}
         \end{aligned}$};
    \node[ellipse, draw=alizarin!120, dashed, thick, left of=output, node distance=4.7cm, align=left, yshift=-0.4cm, minimum height=2mm, minimum width=6mm, inner sep=0, outer sep=0] (una) {};
    \begin{scope}[on background layer]
        \node[draw, fit={([xshift=-1mm, yshift=-1mm] ma.north east) (una)}, dashed, fill=gallery!42, inner sep=0.4em] {};
     \end{scope}
     
     \node[ellipse, draw=alizarin!120, dashed, thick, minimum height=1mm, minimum width=7mm, inner sep=0, outer sep=0, fit={(un_edge)}, rotate=-15] (un) {};
     
     \node[rectangle, fill=alizarin!62, dashed, thick, left of=o, node distance=4.25cm, yshift=0.3cm, inner sep=4, outer sep=1, rounded corners=2] (query) {Unlearning};
     \draw[FARROW, draw=alizarin!120, dashed] (query.north) to [bend left=30] (un.south);
     
     \node [model, fill=alizarin!62, draw=alizarin!120, left of=m1, node distance=1.2cm] (un_m1) {$M_{1}'$};
     
     \draw[FARROW, draw=alizarin!120, dashed]  ($(s1.north)+(-0.2, 0)$) to [bend left] node [pos=0.3, yshift=2mm] {\small $S_{1}'$} (un_m1.south)  ;
     \draw[FARROW, draw=alizarin!120, dashed]  (un_m1.north) to [bend left] (agg.west)  {} ;
    
    \end{tikzpicture}
    }
    \caption{Illustration of our RecEraser framework, which consists of three phases: data partition, shard model training, and shard model aggregation. When receiving an unlearning request of data, only the corresponding shard model needs to retrain.}
\end{figure}




==> rebuttal.tex <==
We thank all reviewers for the valuable reviews and comments. In the following are our responses:

To reviewer #1:

1. We will carefully check and revise our paper to avoid typo errors.

2. Discussions about the unlearning process:
The pretrain embeddings need to be used only once in the data partition part to construct RecEraser. After that, an unlearning operation only needs to retrain the corresponding shard model and the aggregation part. In Table 4, we show that retraining these two parts are much faster than retraining from the original data.

3. How do I know the data is indeed removed:
For approximate unlearning methods, whether the data is removed needs to be measured by experiment since they can't guarantee 100%

We will make corrections and add corresponding analysis in our manuscript according to your comments. 

To reviewer #2:

1. On originality:
In our paper, we have described the SISA model in detail and discussed the differences between RecEraser and SISA: (1) New data partition methods to keep the collaborative information; (2) Adaptive aggregation method to improve the model utility. 

2. Evaluation of recommendation performance:

Our experiments follow the standard settings of recommendation research. We rank all candidate items to calculate the evaluation metrics [1]. Since the target candidate set in recommendation is usually very large, the metric scores are usually much smaller than that in other tasks like text or image classification. In this case, a small improvement could also be very beneficial for real-word recommender systems. Similar results can also be found in many representative recommendation papers [2,3]. 

Moreover, since the Yelp dataset has a larger candidate set than ml-1m (38048 vs. 3706), the metric scores are relatively smaller than those on Movielens. However, our RecEraser can still achieve about 90%

We will add more analysis according to your comments. 

To reviewer #3:

1. Limitations and future work
At present, our RecEraser is limited to the setting where the unlearning requests arrive sequentially. Alternatively, the system can also aggregate several unlearning requests into a batch and then unlearn this batch at once. How to efficiently unlearning in batch setting is still an open problem. 

In the future, we seek to improve the unlearning efficiency in batch setting, we will also try to incorporate the content features of users and items to avoid performance degradation. 
We will add more analysis according to your comments. 

To reviewer #4: 

1. How often one needs to re-split the data into balanced shards:

Our work is based on the assumption that the unlearning request is issued uniformly since we have no prior knowledge about the unlearning request distribution. Under uniform assumption, the size of each shard can maintain the similar size during unlearning procedure. Distribution-aware sharding is an interesting and valuable problem for future work. We will add more discussion about this problem in revision paper.

2. Why using WMF for pretrain:
WMF is a very simple and representative recommendation model and can be trained very quickly as shown in Table 4.

3. How datasets are converted into implicit feedback:
In our experiments, the rating is transformed into implicit based on interaction (not just ratings of 4s and 5s). This is a widely used pre-processing method [2,3]. In implicit setting, recommendation task is to predict whether a user will interact with an item (like click), not to predict ratings. From this perspective, the above data pre-processing method is also reasonable.

4. Hyper-parameter settings:
Common hyper-parameters like batch size and embedding size are the same for all base models. For model-specific hyper-parameters, like dropout and GNN layers, we tune them in the ranges suggested by their original papers.

5. On suggestions:
Thanks for your suggestions! In the future we are also interested in beyond-accuracy metrics such as diversity and fairness. For "model-agnostic", we will make it more clear by changing it to "the architecture of RecEraser is model-agnostic for base models that can create latent representations of users and items". For the number of shards, it is set to 10 in our main experiments (Table 3) to ensure each shard is trained on a reasonable number of interactions. 

We will add more analysis to our paper according to your suggestions.

[1] Walid Krichene et al. On Sampled Metrics for Item Recommendation. KDD 2020.
[2] Xiangnan He, et al. LightGCN: Simplifying and Powering Graph Convolution Network for Recommendation. SIGIR 2020.
[3] Chong Chen, et al. Efficient Neural Matrix Factorization without Sampling for Recommendation. TOIS 2020.







